Reinforcement Learning for Efficient Returns Management

In retail warehouses, returned products are typically placed in an intermediate storage until a decision regarding further shipment to stores is made. The longer products are held in storage, the higher the inefficiency and costs of the returns management process, since enough storage area has to be provided and maintained while the products are not placed for sale. To reduce the average product storage time, we consider an alternative solution where reallocation decisions for products can be made instantly upon their arrival in the warehouse allowing only a limited number of products to still be stored simultaneously. We transfer the problem to an online multiple knapsack problem and propose a novel reinforcement learning approach to pack the items (products) into the knapsacks (stores) such that the overall value (expected revenue) is maximized. Empirical evaluations on simulated data demonstrate that, compared to the usual offline decision procedure, our approach comes with a performance gap of only 3% while significantly reducing the average storage time of a product by 96%.

==> mybibfile_template.tex <==
@article{turing1950computing,
    author = {Turing, Alan M.},
    title = {Computing Machinery and Intelligence},
    journal = {Mind},
    volume = {LIX},
    number = {236},
    pages = {433--460},
    year = {1950}
}

@article{rumelhart1986learning,
  title = {Learning Representations by Back-Propagating Errors},
  author = {Rumelhart, David E. and Hinton, Geoffrey E. and Williams, Ronald J.},
  journal = {Nature},
  volume = {323},
  number = {6088},
  pages = {533--536},
  year = {1986}
}

@inproceedings{kautz1992planning,
  title = {Planning as Satisfiability},
  author = {Kautz, Henry A. and Selman, Bart},
  booktitle = {Proceedings of the 10th European Conference on Artificial Intelligence (ECAI)},
  pages = {359--363},
  year = {1992}
}



@article{grosz1996collaborative,
  title = {Collaborative Plans for Complex Group Action},
  author = {Grosz, Barbara J. and Kraus, Sarit},
  journal = {Artificial Intelligence},
  volume = {86},
  number = {2},
  pages = {269--357},
  year = {1996}
}

@misc{perelman2002entropy,
  title = {The Entropy Formula for the {R}icci Flow and its Geometric Applications}, 
  author = {Grisha Perelman},
  howpublished = {Preprint arXiv:math/0211159},
  year = {2002}
}

@book{pearl2009causality,
  title = {Causality},
  author = {Pearl, Judea},
  publisher = {Cambridge University Press},
  year = {2009}
}


